An Algorithm for Multi-Attribute Diverse Matching

Bipartite b-matching, where agents on one side of a market are matched to one or more agents or items on the other, is a classical model that is used in myriad application areas such as healthcare, advertising, education, and general resource allocation. Traditionally, the primary goal of such models is to maximize a linear function of the constituent matches (e.g., linear social welfare maximization) subject to some constraints. Recent work has studied a new goal of balancing whole-match diversity and economic efficiency, where the objective is instead a monotone submodular function over the matching. Basic versions of this problem are solvable in polynomial time. In this work, we prove that the problem of simultaneously maximizing diversity along several features (e.g., country of citizenship, gender, skills) is NP-hard. To address this problem, we develop the first combinatorial algorithm that constructs provably-optimal diverse b-matchings in pseudo-polynomial time. We also provide a Mixed-Integer Quadratic formulation for the same problem and show that our method guarantees optimal solutions and takes less computation time for a reviewer assignment application.

==> On Diverse Bipartite b-Matchings/abstract.tex <==
Bipartite $b$-matching, where agents on one side of a market are matched to one or more agents or items on the other, is a classical model that is used in myriad application areas such as healthcare, advertising, education, and general resource allocation. Traditionally, the primary goal of such models is to maximize a linear function of the constituent matches (e.g., linear social welfare maximization) subject to some constraints. Recent work has studied a new goal of balancing whole-match \emph{diversity} and economic efficiency, where the objective is instead a monotone submodular function over the matching.  Basic versions of this problem are solvable in polynomial time. In this work, we prove that the problem of simultaneously maximizing diversity along several features (e.g., country of citizenship, gender, skills) is NP-hard. To address this problem, we develop the first combinatorial algorithm that constructs provably-optimal diverse $b$-matchings in pseudo-polynomial time. We also provide a Mixed-Integer Quadratic formulation for the same problem and show that our method guarantees optimal solutions and takes less computation time for a reviewer assignment application. 
%We then compare directly, on real-world datasets, against the state-of-the-art, quadratic-programming-based approach to solving diverse $b$-matching problems and show that our method outperforms it in both speed and (anytime) solution quality.



% In this work, we identify theoretically-tractable segments of the diverse $b$-matching problem space and propose new algorithms that construct provably-optimal diverse $b$-matchings in pseudo-polynomial time.  

==> On Diverse Bipartite b-Matchings/algorithm.tex <==
\section{Negative-Cycle-Detection-based Algorithms}
\label{algorithm}
%\saba{Mention $T_0$ is different with the other teams.}

In this section, we explain our algorithm for finding the optimum assignment. First, we build an auxiliary graph $G'$. For each team $T_i$, there is a switch in $G'$ with $|\mathcal{V}|$ input ports, and $|\mathcal{V}|$ output ports, where $|\mathcal{V}|$ is the number of columns in the matrix representation. Each port is a node in $G'$, and each switch is a directed bipartite graph, with edges going from its input ports (nodes) to its output ports. In Figure~\ref{fig:graph-exchange}, each box is a switch.
A dummy team $T_0$ is introduced to accommodate all unassigned workers in the matching.
Inside a switch $T_i$, there is a directed edge from each input port to each output port. If the directed edge is connecting two ports such that their corresponding combinations of features do not have the same value for any features, the weight of this edge is equal to zero. Otherwise, per each feature $f_k$ that has the same value, $-2\lambda_k$ is added to the weight of this edge.
%For each pair of input output ports $(I_{j_1}^i, O_{j_2}^i)$ in switch $T_i$, there is a directed edge $e_{j_1, j_2}^i$ from $I_{j_1}^i$ to $O_{j_2}^i$, its weight is defined in the following way:
%\[ w(e_{j_1, j_2}^i)=\begin{cases} 
%      -2\lambda_1 & \text{if } j_1 = j_2, i\neq 0 \\
%      0 & \text{o.w}
%   \end{cases}
%\]

The reason behind assigning these weights to the edges is to make sure in a local exchange, considering a fixed feature $f_k$, the nodes which are not a source-transition or a sink-transition w.r.t. $M_{k}$, have zero contribution to $\Delta(D_k)$.
%The reason behind putting the weight of edges in the first case equal to $-2\lambda_1$ is to force the nodes which are not a source-transition or a sink-transition and do not belong to $T_0$, to have zero contribution to gain of a cycle. 

For each pair of teams $T_{i_1}$ and $T_{i_2}$ where ${i_1}\neq {i_2}$, and for each feature combination $v_j$, there is a directed edge from output port $O_{j}^{i_1}$ of switch $T_{i_1}$ to the input port $I_{j}^{i_2}$ of switch $T_{i_2}$, and weight of this edge captures the difference in the objective function when in the matrix representation a person in column $V_j$ (with feature set $v_j$) is moved from $T_{i_1}$ to $T_{i,2}$. 
% \saba{I dropped the formal definition of weights to save space.}

%Let's assume $v_j = (f_{1,k'_1},\cdots, f_{|\mathcal{F}|, k'_{\mathcal{F}}})$, then:
%\[\begin{cases}
%    \sum_{k=1}^{|\mathcal{F}|}\lambda_k\Big((c_{{i_2},k,k'_k}+1)^2 - c^2_{{i_2},k, k'_k} + (c_{{i_1},k, k'_k}-1)^2 -
%    \\
%    \quad c^2_{{i_1},k,k'_k}\Big)  + \big( u_{{i_2},k'_1}-u_{{i_1},k'_1}\big) & {i_1},{i_2}\neq 0\\
%    \sum_{k=1}^{|\mathcal{F}|}\lambda_k\Big((c_{{i_2},k,k'_k}+1)^2 - c^2_{{i_2},k, k'_k} \Big)  + \big( u_{{i_2},k'_1}\big) & {i_1}=0\\
%    \sum_{k=1}^{|\mathcal{F}|}\lambda_k\Big( (c_{{i_1},k, k'_k}-1)^2 - c^2_{{i_1},k,k'_k}\Big)  + \big( -u_{{i_1},k'_1}\big) & {i_2}=0\\
%    \end{cases}
%\]

%There are separate cases for ${i_1}~or~{i_2}~=~0$ since $T_0$ is a node corresponding to a dummy team, which is allocated all the unassigned workers from each country. The contribution of this team to the objective function must be zero.

Each cycle in this graph is corresponding to a cycle in a matrix representation and local exchanges along them have the same gain. Figure~\ref{fig:graph-exchange} shows a cycle which is corresponding to the cycles in Figures~\ref{fig:matrix-exchange} and~\ref{fig:matching-exchange}.% In this cycle, weight of edges is defined in the following:
%$e_1$ denoted by $w(e_1)$ is equal to $0$, also:
%\begin{align*}
%&w(e_1) = w(e_5) = 0\\
%&w(e_2) = \lambda_1\big((c_{2,1}+1)^2 - c^2_{2,1} + (c_{1,1}-1)^2 - c^2_{1,1}\big) +\\ &\qquad\lambda_2\big(u_{2,1}-u_{1,1}\big)\\
%&w(e_3)=-2\lambda_1\\
%&w(e_4) = \lambda_1\big((c_{3,1}+1)^2 - c^2_{3,1} +(c_{2,1}-1)^2 - c^2_{2,1}\big) +\\ &\qquad\lambda_2\big(u_{3,1}-u_{2,1}\big)\\
%&w(e_5)=0\\
%&w(e_6)=\lambda_1\big((c_{1,2}+1)^2 - c^2_{1,2} + (c_{3,2}-1)^2 - c^2_{3,2}\big) +\\
%&\qquad\lambda_2\big(u_{1,2}-u_{3,2}\big)
%\end{align*}




%%FA notes on notation used
%% for each edge in auxilary graph, there are five parameters
%% Team i, country of edge origin j (output or not ) , country of edge end k (input or not) 
%% C is redefined as a negative cycle. small c also represents a cycle. U is defined twice as minimum weight of matching and total utility.

After constructing the auxiliary graph, we run Algorithm~\ref{alg-neg-cycle-detection}. 
Algorithm~\ref{alg-neg-cycle-detection} moves workers from one team to another if it detects a negative cycle. %The movement of a worker is always from an output port of a team to an input port of another team.

\begin{algorithm}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Directed weighted graph $G'$, initial feasible $b$-matching $Q$ which satisfies team demands.}
\Output{Optimal diverse $b$-matching}

 \While{$\exists$ a negative cycle $C\in G'$}{
  // Perform a local exchange operation along $C$\;
  \For{$e\in C$}{
    // Assume edge $e$ is from output port $O_{j}^{i_1}$ of team $T_{i_1}$ to input port $I_{j}^{i_2}$ of another team $T_{i_2}$\;
    // Move one worker with feature set $v_j = \{f_{1,k'_1}, \cdots, f_{|\mathcal{F}|, k'_{|\mathcal{F}|}}\}$ from team $T_{i_1}$ to team $T_{i_2}$:\\
    $\forall k\in \{1,\cdots, |\mathcal{F}|\}$:
    $c_{i_1,k,k'_k}-=1, c_{i_2,k,k'_k}+=1$\;
    %$c_{i_2,k,k'_k}+=1$\;
    Update weight of edges of $G'$ w.r.t to the new values of $c_{i_1,k,k'_k}$, and $c_{i_2,k,k'_k}$\;
  }
 }
 \caption{Find optimal diverse $b$-matching}
  \label{alg-neg-cycle-detection}
\end{algorithm}
Algorithm~\ref{alg-neg-cycle-detection} takes as input an initial feasible solution $Q$ as input. To find $Q$, we first find a feasible solution, which satisfies all the demand constraints. 
In order to find an initial feasible solution, in each iteration, consider the first subset of workers in the the bipartite graph G ($V_j$) with at least one un-assigned worker, and the first team ($T_i$) such that the number of workers assigned to it is less than its demand (In the first iteration, we start with $V_1, T_1$, and all the workers are un-assigned). 
Assign un-assigned workers from $V_j$ to $T_i$, until either demand of $T_i$ is fully satisfied, in this case, move to the next team $(i=i+1)$, or all the workers from $V_j$ are assigned, then let $j=j+1$. Repeat this procedure until all the demand constraints are satisfied. Time complexity of this procedure is $\mathcal{O}(|\mathcal{V}|+t)$.
%We can also initialize it with the minimum weight solution, which also serves the purpose of a baseline. We compare the final diversity by diverse matching method to the initial diversity of this solution. 

In Algorithm~\ref{alg-neg-cycle-detection}, any negative cycle detection algorithm can be used to detect negative cycles in $G'$. We use a heuristic improvement of Bellman-Ford proposed by Goldberg and Radzik~\cite{Goldberg93aheuristic} in our experiments.
\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth, scale = 0.5]{figures/IJCAI-pic3v3.pdf}
    \caption{A local Exchange in graph representation. %The edge weights are $w(e_1) = w(e_5) = -2\lambda_1$, $w(e_2) = \lambda_0\big(u_{2,1}-u_{1,1}\big) +\lambda_1\big((c_{2,1,1}+1)^2 - c^2_{2,1,1} +  (c_{1,1,1}-1)^2 - c^2_{1,1,1} \big) +\lambda_2\big((c_{2,2,1}+1)^2 - c^2_{2,2,1} + (c_{1,2,1}-1)^2 - c^2_{1,2,1}\big), w(e_3)=-2\lambda_1-2\lambda_2$, $w(e_4) =
    %\lambda_0\big(u_{3,1}-u_{2,1}\big)+\lambda_1\big((c_{3,1,1}+1)^2 - c^2_{3,1,1} +(c_{2,1,1}-1)^2 - c^2_{2,1,1}\big) +
    %\lambda_2\big((c_{3,2,1}+1)^2 - c^2_{3,2,1} +(c_{2,2,1}-1)^2 - c^2_{2,2,1}\big)$, $w(e_6)=\lambda_0\big(u_{1,2}-u_{3,2}\big)+\lambda_1\big((c_{1,1,1}+1)^2 - c^2_{1,1,1} + (c_{3,1,1}-1)^2 - c^2_{3,1,1}\big) + \lambda_2\big((c_{1,2,2}+1)^2 - c^2_{1,2,2} + (c_{3,2,2}-1)^2 - c^2_{3,2,2}\big)
    %$
    }
    \label{fig:graph-exchange}
\end{figure}

==> On Diverse Bipartite b-Matchings/analysis.tex <==
\section{Proof of Optimality}
In this section, % in Theorem~\ref{proof-correctness},
we prove that Algorithm~\ref{alg-neg-cycle-detection} gives the optimum solution for diverse bipartite $b$-matching problem. 

Assume after the algorithm ends, the final assignment is a local optimum $P$, and the optimum solution is $P^*$. 
Consider the matching representations of $P$ and $P^*$. The symmetric difference of $P$ and $P^*$ ($P\oplus P^*$) can be decomposed into a set of alternating cycles and paths of even length. The reason that the length of alternating paths is even is that size of both of the matchings is equal: $|P| = |P^*|=\sum_{i=1}^t d_i$.

Each local exchange along an alternating cycle corresponds to a cycle in the matrix representation. A local exchange along an alternating path corresponds to a cycle in a matrix representation which includes vertices from row $T_0$. 
%\saba{I'm dropping the example here, to save some space.}
%For example, Figure~\ref{fig:alternating-path} shows a local exchange along an alternating path in $M\oplus M^*$ where red edges belong to $M^*$, and black edges belong to $M$. Matrix representation corresponding to this local exchange is shown in Figure~\ref{fig:path-exchange-matrix}.

%\begin{figure}
%    \centering
%        \includegraphics[width=0.3\textwidth]{figures/IJCAI-pic8v2.png}
%    \caption{Example of a local exchange along an alternating path.}
%    \label{fig:alternating-path}
%\end{figure}


%\begin{figure}
%    \centering
%    \includegraphics[width=0.25\textwidth, ]{figures/IJCAI-pic7v2.png}
%    \caption{Matrix representation showing an alternating path.}
%    \label{fig:path-exchange-matrix}
%\end{figure}

Before proving Thm.~\ref{proof-correctness}, we need the following definitions:

\textbf{Maximal Cycle:} A cycle $y$ in a matrix representation $M$ is maximal if its source-transitions (nodes with zero incoming edges) and sink-transitions (nodes with zero outgoing edges) are source-transition and sink-transition w.r.t all the edges in %$M\oplus M^*$ 
$M$ as well. For example, consider Figure~\ref{fig:maximal-cycle}. Let's call the green cycle $y_g$, the red cycle $y_r$, and the blue cycle $y_b$.
The $y_g$ has two source-transitions $w_{1,1}, w_{0,3}$, and it has two sink-transitions $w_{0,1}, w_{1,3}$. Since there are no edges going out of $w_{1,3}, w_{0,1}$, and no edges going into $w_{0,3}, w_{1,1}$, $y_g$ is a maximal cycle. Cycles $y_r, y_b$ are maximal cycles as well. Therefore, $\{y_g\cup y_b\cup y_r\}$ gives a maximal cycle decomposition for $M$. However, if we consider embedding of $M$ w.r.t gender ($M_2$), then $y_r$ is not a maximal cycle anymore, and $\{y_g, y_r \cup y_b\}$ gives a maximal cycle decomposition w.r.t $M_2$ and $M_1$(embedding w.r.t countries).
A cycle is called all-maximal cycle if it is maximal w.r.t all the matrix representations $M_{1}, \cdots, M_{|\mathcal{F}|}$. In this example, $\{y_g, y_r \cup y_b\}$ gives an all-maximal cycle decomposition.
%is not a maximal cycle since $c_{2,2}$ is a source-transition w.r.t the red edges, but it is not a source-transition w.r.t all edges and a blue edge is going into it. Also $c_{2,1}$ is a sink-transition w.r.t the red edges, but there is a blue edge going out of it. Cycle $c_b$ is not a maximal cycle as well.


\begin{figure}
    \centering
    \includegraphics[width=0.35\textwidth]{figures/IJCAI-pic6v4.png}
    \caption{Maximal cycle decomposition}
    \label{fig:maximal-cycle}
\end{figure}
\begin{lemma}
The set of all the edges of $P\oplus P^*$ can be decomposed into a set of all-maximal cycles.
\end{lemma}
\begin{proof}
Consider an arbitrary decomposition of the edges of $P\oplus P^*$ in the matrix representation into a set of cycles $\{y_1,\cdots,y_{\ell}\}$.
If there exists a cycle in $P\oplus P^*$ without any source-transitions and sink-transitions, it means the gain of this cycle is zero and it could be discarded. If there exists any cycle $y_p$ which is not all-maximal, then there exists another cycle $y_q$ which makes $y_p$ not to be maximal w.r.t some features. For example in Figure~\ref{fig:maximal-cycle}, $y_r$ is not maximal because of $y_b$. In this case, union $y_p$ and $y_q$, and make $y_p\cup y_q$ a single cycle in the decomposition. At the end, all the edges in $P\oplus P^*$ will be decomposed into a set of all-maximal cycles. Let's call the set of all-maximal cycles $\{y'_1,\cdots, y'_{\ell'}\}$.
\end{proof}
%For example, in Figure~\ref{fig:maximal-cycle}, decomposition $\{c_g, c_r\cup c_b\}$ is a maximal cycle decomposition. Now we are ready to prove the following theorem:
\begin{theorem}
\label{proof-correctness}
Algorithm~\ref{alg-neg-cycle-detection} finds the global optimum for the diverse $b$-matching problem.
\end{theorem}
%the negative cycle detection algorithm finds the global optimum.
\begin{proof}
Let $f(P)$ show the value of the objective function for the assignment $P$. $f(P^*)-f(P)<0$ therefore:
\scriptsize{\[{f(P^*)-f(P) = gain(y'_{1,1}) + gain(y'_{2,2})+\cdots
+gain(y'_{\ell', \ell'}) < 0}\]
}
\normalsize{}
Where $y'_k$ ($1\leq k \leq \ell'$) is the $k^{th}$ cycle in the maximal cycle decomposition, and $y'_{k,k}$ is applying the local exchange of the cycle $y'_{k}$ at step $k$. The initial step is the assignment $P$. Since $f(P^*)-f(P)<0$, there must be a maximal cycle $y'_g$ such that $gain(y'_{g,g})<0$. We wish to show $gain(y'_{g,1})<0$, which implies starting from the initial assignment $P$, a local exchange can be done with a negative gain, and $P$ is not a local optimum which is a contradiction.

Let $D(y'_{g,g}), U(y'_{g,g})$ denote respectively the change in the diversity, and the change in the utility when applying a local exchange $y'_{g}$ in step $g$.
Let $D_{f_k}(y'_{g,g})$ denote the change in the diversity w.r.t the feature $f_k$, when applying $y'_{g,g}$. Therefore:
\[gain(y'_{g,g}) = \sum_{k\in |\mathcal{F}|} D_{f_k}(y'_{g,g}) + U(y'_{g,g})\]
Lemma~\ref{upper-bound-diversity-one-feature} shows if $D_{f_k}(y'_{g,g}) < 0$, then $D_{f_k}(y'_{g,1}) < 0$.
As a result, $D(y'_{g,g}) < 0$ implies $D(y'_{g,1}) < 0$. It is easy to see that $U(y'_{g,g}) = U(y'_{g,1})$. Therefore, $gain(y'_{g,g})<0$ implies $gain(y'_{g,1}) < 0$, and the proof is complete.
\end{proof}
\begin{lemma}\label{upper-bound-diversity-one-feature} If $D_{f_k}(y'_{g,g}) < 0$, then $D_{f_k}(y'_{g,1}) < 0$.
\end{lemma}
\begin{proof}
Consider $y'_{g,g}$ embedded into $M_{k}$. There are four types of vertices in $y'_{g,g}$:
\begin{itemize}
   \item Vertices in the form of $w_{0,j}$  where $1\leq j\leq |\mathcal{V}|$. These vertices have contribution zero to both $D_{f_k}(y'_{g,g})$ and $D_{f_k}(y'_{g,1})$.
   \item Vertices that are not sink-transition or source-transition, i.e. $w_{2,2}$ in Figure~\ref{fig:matrix-exchange}, w.r.t $M_k$. It could be seen that contribution of these nodes to both $D_{f_k}(y'_{g,g})$ and $D_{f_k}(y'_{g,1})$ is zero.
   \item Sink-transitions: Consider an arbitrary sink-transition $v$ in $y'_{g,g}$. Assume the value of this node at the beginning of step $g$ is $v_g$. The contribution of $v$ to $D_{f_k}(y'_{g,g})$ is $\lambda_k\big((v_g+1)^2 - v_g^2\big)>0$. Since $v$ is a sink-transition, $v_g\geq v_1$. Therefore, $\lambda_k\big((v_g+1)^2 - v_g^2\big)\geq\lambda_k\big( (v_1+1)^2 - v_1^2\big)$.% As a result, the contribution of $v$ to $D_{f_k}(y'_{g,1})$ is upper bounded by its contribution to $D_{f_k}(y'_{g,g})$.
   \item Source-transitions: Consider an arbitrary source-transition $v$ in $y'_{g,g}$. %Assume the value of this node at the beginning of step $g$ is $v_g$. 
   The contribution of $v$ to $D_{f_k}(y'_{g,g})$ is $\lambda_k\big((v_g-1)^2 - v_g^2\big)$. Since $v$ is a source-transition $v_1\geq v_g$, and therefore $\lambda_k\big((v_g-1)^2-v_g^2\big) \geq \lambda_k\big((v_1-1)^2 - v_1^2\big)$.
\end{itemize}
At the end, contribution of all the vertices to $D_{f_k}(y'_{g,1})$ is upper bounded by their contribution to $D_{f_k}(y'_{g,g})$. Therefore if $D_{f_k}(y'_{g,g})<0$, then $D_{f_k}(y'_{g,1})<0$.
\end{proof}
\begin{theorem}
\label{thm:running-time}
The running time of the algorithm is $\mathcal{O}((\lambda_{\max}\cdot|\mathcal{F}|\cdot n^2+\lambda_0U)\cdot |\mathcal{V}|^2\cdot t^2(|\mathcal{V}|+t))$, where $U$ is the maximum cost of an initial feasible b-matching and $\lambda_{max} = \max\{\lambda_1,\cdots, \lambda_{|\mathcal{F}|}\}$.
\end{theorem}
In order to prove this theorem, first we show the following lemmas hold.
\begin{lemma}
\label{lem:num-iter}
The number of iterations of our algorithm is at most $(\lambda_{max}\cdot|\mathcal{F}|\cdot n^2 + \lambda_0 U)$.
\end{lemma}
\begin{proof}
The initial state of the algorithm is a feasible b-matching with cost at most $U$. Diversity of any matching is at most $\lambda_{max}\cdot|\mathcal{F}|\cdot n^2$. At each iteration, we find a negative weight cycle and since all the weights are integers, its weight can be at most $-1$. Therefore, the objective function decreases by at least $1$ at each step, and since the value of the objective function is always positive, the number of iterations is at most $(\lambda_{max}\cdot|\mathcal{F}|\cdot n^2 + \lambda_0 U)$.
\end{proof}
\begin{lemma}
\label{lem:complexity-bellman-ford}
The complexity of each iteration of the algorithm is $\mathcal{O}(|\mathcal{V}|^2\cdot t^2(|\mathcal{V}|+t))$.
\end{lemma}
\begin{proof}
At each iteration, we use a negative cycle detection algorithm with running time $\mathcal{O}(|V|\cdot |E|)$ (where $|V|$ is the number of nodes in the auxiliary graph and $|E|$ is the number of edges). The number of nodes in the graph is $2|\mathcal{V}|\cdot (t+1)$, since there are $t+1$ switches in the graph and each switch has exactly $2|\mathcal{V}|$ ports and each port is a node in the graph. The number of edges incident on each port is $|\mathcal{V}|+t$. Therefore, the total number of edges is $\mathcal{O}(|\mathcal{V}|\cdot t(|\mathcal{V}|+t))$. Hence, the complexity of each iteration is $\mathcal{O}(|\mathcal{V}|^2\cdot t^2(|\mathcal{V}|+t))$.
\end{proof}
Combining Lemma~\ref{lem:num-iter} with Lemma~\ref{lem:complexity-bellman-ford}, and considering $\mathcal{O}(|\mathcal{V}|+t)$ time complexity for finding an initial feasible solution, yields Theorem~\ref{thm:running-time}.

==> On Diverse Bipartite b-Matchings/conclusion.tex <==
\section{Conclusion \& Future Research}\label{sec:conclusions}

In this paper, we proposed the first pseudo-polynomial time algorithms for multi-feature diverse weighted bipartite $b$-matching---a problem that we also showed is NP-hard. We propose an algorithm that not only guarantees an optimal solution but also converges faster than a proposed approach using a black-box industrial MIQP solver. We demonstrated our results on a dataset for paper reviewer matching. Future work could explore the extension of this method to online diverse matching~\cite{Dickerson19:Balancing}, where vertices arrive sequentially and must match immediately; this has direct application in advertising, where one could balance notions of reach, frequency, and immediate monetary return.  Exploring connections to fairness in machine learning~\cite{Grgic-Hlava18:Beyond} and hiring~\cite{Schumann19:Diverse} by way of diversity are also of immediate interest.

==> On Diverse Bipartite b-Matchings/experiments.tex <==
\section{Experimental Validation \& Discussion}\label{sec:experiments}
To demonstrate the efficacy of the proposed method, we apply it to a dataset of reviewer paper matching. First, we find the optimal solution for multi-feature reviewer paper matching and compare it to the single feature diverse matching method. We also provide the MIQP formulation of the same problem based on literature and show how our algorithm is faster to the Gurobi based MIQP solver.

%\subsection{Application to Reviewer Assignment}
%In this section, we solve the reviewer assignment problem, where each reviewer has multiple features. 
For the reviewer assignment problem, where each reviewer has multiple features, we want to match each paper with reviewers who are not only from different expertise areas (clusters), but also belong to different genders. We use the multi-aspect review assignment evaluation dataset~\cite{karimzadehgan2009constrained}, a benchmark dataset from UIUC. It contains $73$ papers accepted by SIGIR $2007$, and $189$ prospective reviewers who had published in the main information retrieval conferences. The dataset provides $25$ major topics and for each paper in the set, an expert provided $25$-dimensional label on that paper based on a set of defined topics. Similarly for the $189$ reviewers, a $25$-dimensional expertise representation is provided. 

% We use Algorithm~\ref{alg-neg-cycle-detection} for diverse matching problem to determine the most appropriate reviewers for a manuscript by also ensuring that reviewers are different from each other. 
To compare our method (Algorithm~\ref{alg-neg-cycle-detection}) with a baseline, we formulate a multi-feature MIQP variant of our problem, which is an extension of the single-feature formulation provided in~\cite{Ahmed:2017:DWB:3171642.3171649} and is given by:
\begin{align*}
&\min\lambda_0\sum_{i=1}^t \sum_{j=1}^{|\mathcal{F}_1|} u_{i,j}\cdot c_{i,1,j}+\sum_{k=1}^{|\mathcal{F}|} \lambda_k \sum_{i=1}^t\sum_{k'=1}^{|\mathcal{F}_k|}c_{i,k,k'}^2\\
& \sum_{k=1}^{|\mathcal{F}|}\sum_{k'=1}^{|\mathcal{F}_k|} c_{i,k,k'} = d_i, \forall 1\leq i\leq t\\
&\sum_{i=0}^t c_{i,k,k'} = |\mathcal{F}_{k,k'}|, 1\leq k\leq |\mathcal{F}|,1\leq k' \leq |\mathcal{F}_{k}|
\end{align*}
To set up the graph for our method, we first cluster the reviewers into $5$ clusters based on their topic vectors using spectral clustering. To calculate the relevance of each cluster for any paper, we take the average cosine similarity of label vectors of reviewers in that cluster and the paper. We set the constraints such that each paper matches with exactly $4$ reviewers, and no reviewer is allocated more than $1$ paper. To increase dataset size, we double the number of reviewers by creating a copy of each reviewer. As the original dataset lacks gender information, we added a new feature to each reviewer in this dataset by randomly adding one of two gender labels (Male or Female) to each reviewer. We set $\lambda_0 = \lambda_1 = \lambda_2 = 1 $ for our experiments. 


%We need to double the number of reviewers in each cluster to make sure the total demand of the papers could be satisfied.

 %We show that our method discussed in Section~\ref{sec:multi-attributes} finds the optimum solution. We further validated it against MIQP formulation of the same problem.
 
%\subsection{Experimental Validation for Workers with Multiple Features}
%In this section, we discuss the importance of workers with multiple features. 
%In Section~\ref{sec:experiments}, we demonstrated how diverse matching methods can help obtain solutions for the paper reviewer assignment problem.
%Each reviewer belonged to one of five clusters and the goal was to match a paper with reviewers from different clusters. By varying a diversity parameter, we obtain the entire trade-off front between diversity and total cost of the matching.



%$\lambda_{g}$ controls how much weight we assign to gender diversity and $\lambda_{c}$ is the weight assigned to country diversity.  $|S_{T_i, C_j, G_g}|$ is the number of workers from country $j$ and gender $g$ assigned to team $T_i$. The objective function is equal to $\sum_{i=1}^t f(T_i)$.

%To demonstrate our algorithm, we solve this problem using both MIQP and our auxiliary graph method. We demonstrate our method on the modified UIUC dataset used in Section~\ref{sec:experiments}. %with 73 papers and 378 reviewers. Each paper needs exactly 4 reviewers and each reviewer can review maximum two papers.


We run the negative cycle detection algorithm, and the MIQP solver using Gurobi to find the optimum solution. 
On converging to the optimal solution, we find that all $73$ papers receive two male reviewers and two female reviewers, which shows that the method was capable of balancing gender diversity. All papers receive reviewers from four different clusters too. If we only optimize for cluster diversity, it is possible that the gender ratio for individual paper gets skewed. When we run the same model with $\lambda_{g}=0$ (no weight to gender diversity), we find that out of $73$ papers, $12$ papers receive all four reviewers of the same gender and $41$ papers receive three reviewers of the same gender. Hence, only $27.3\%$ teams of reviewers are gender balanced. However, one should note that when we do not keep gender as an objective, the resultant allocation is random and different skewness can be observed in different runs based on the initial solution. 

Finally, we compare the timing performance of our algorithm with MIQP by changing the number of papers that need to be reviewed on a Dell XPS 13 laptop with i7 processor. For MIQP, we set a maximum run time of four hours (14400 seconds) for Gurobi solver, at which we report the current best MIQP solution.
Table~\ref{tab:res} shows that for all cases with the number of papers greater than $13$, MIQP does not converge within four hours, while our method finds the optimum solution in lesser time. Interestingly, MIQP current solutions are found to be the same as the optimum solution found by our method, which shows that for this application, MIQP was able to search the solution but it was not able to prove that the solution is optimum. In contrast, our method finds the solution faster as well as guarantees that it is optimum. %The timing performance of our algorithm can be further improved by finding negative cycles in parallel and optimizing the code. 


\begin{table}[!htbp]
\scriptsize
\centering
\begin{tabular}{rrrr}
\toprule
%Number of movies & MIQP Time & Our Method Time & MIQP Objective & Our Method Objective & WBM Objective\\
\# Papers & \# Reviewers & MIQP Time (s) & Our Method Time (s)\\
\midrule
% 03 & 80 & 24.68 & 0.18\\
% 13 & 280 &  3979.90 & 14.84\\
% 23 & 480 &  14400.00 & 122.96\\
% 33 & 680 &  14400.00 & 400.56\\
% 43 & 880 &  14400.00 & 825.95\\
% 53 & 1080 &  14400.00 & 2837.15\\
% 63 & 1280 &  14400.00 & 5453.58\\
% 73 & 1480 &  14400.00 & 11040.55\\
03 & 378 & 24.68 & 0.18\\
13 & 378 &  3979.90 & 14.84\\
23 & 378 &  14400.00 & 122.96\\
33 & 378 &  14400.00 & 400.56\\
43 & 378 &  14400.00 & 825.95\\
53 & 378 &  14400.00 & 2837.15\\
63 & 378 &  14400.00 & 5453.58\\
73 & 378 &  14400.00 & 11040.55\\
\bottomrule\\
\end{tabular}
\caption{Comparison of MIQP and our method for UIUC reviewer dataset with each paper needing 4 reviewers.}
\label{tab:res}
\end{table}

% \subsection{Application to Reviewer Assignment}
% We now present an application of Algorithm~\ref{alg-neg-cycle-detection} for diverse matching problem to automatically determine the most appropriate reviewers for a manuscript by also ensuring that reviewers are different from each other. We use the multi-aspect review assignment evaluation dataset~\cite{karimzadehgan2009constrained}, a benchmark dataset from UIUC. It contains $73$ papers accepted by SIGIR $2007$, and $189$ prospective reviewers who had published in the main information retrieval conferences. The dataset provides $25$ major topics and for each paper in the set, an expert provided $25$-dimensional label on that paper based on a set of defined topics. Similarly for the $189$ reviewers, a $25$-dimensional expertise representation is provided.

% To set up the graph, we first cluster the reviewers into $5$ clusters based on their topic vectors using spectral clustering. To calculate the relevance of each cluster for any paper, we take the average cosine similarity of label vectors of reviewers in that cluster and the paper. We set the constraints such that each paper matches with exactly $4$ reviewers, and no reviewer is allocated more than $1$ paper. We need to double the number of reviewers in each cluster to make sure the total demand of the papers could be satisfied.


% We first find a minimum cost (maximum weighted) matching for this problem using the Gurobi Integer Linear Program solver (ILP for finding a maximum weighted bipartite matching is explained in the supplementary material). The resultant matching is found to be non-diverse. All 73 papers are allocated three reviewers who are all from the same cluster. This gives the resultant matching zero average diversity, as measured by Shannon entropy.
% Using the graph algorithm, we show that by varying $\lambda$, we can obtain the trade-off between cost and diversity. 
% Figure~\ref{fig:tradeoff} shows the trade-off front between average Shannon entropy and the total weight of the matching for different values of $\lambda$. For this problem, once $\lambda$ is greater than 0.26, all matchings are maximum diversity matching and they result in the same matching allocation. 

% The trade-off front allows us to understand the impact of diversity on the total cost of the matching for any given domain. For instance, in Fig.~\ref{fig:tradeoff}, by marginally increasing $\lambda$ above 0, we see a large gain in entropy with little loss in the total cost of the matching. This shows that we can greatly increase diversity at little cost to matching efficiency. In the subsequent sections, we set $\lambda=1$ fixed. 

% To demonstrate the efficacy of our algorithm for the case when reviewers have multiple features (like cluster assignment and gender), we ran additional experiments with a modified version of this dataset (by randomly adding genders to each reviewer). We showed that our method discussed in Section~\ref{sec:multi-attributes} finds the optimum solution. We further validated it against MIQP formulation of the same problem, which is discussed in the supplementary material.

% \begin{figure}
%     \centering
%     \includegraphics[width=0.35\textwidth]{figures/uiuc_trade.eps}
%     \caption{Trade-off front between cost and entropy}
%     \label{fig:tradeoff}
% \end{figure}
    
    
% \subsection{Application to MovieLens Data}
% In this section, we compare our negative cycle detection algorithm for the first variation of diverse matching that we discussed, with the MIQP approach in~\cite{Ahmed:2017:DWB:3171642.3171649} with increasing size of the graph. This example considers matching movies to users while ensuring that the movies contain diverse genres. We use a subset of the MovieLens 1M dataset~\cite{harper2016movielens}, which includes one million ratings by 6,040 users for 3,900 items. This dataset contains both users' movie ratings between 1 and 5 and genre categories for each movie (\eg, comedy, romance, and action). We first train a standard collaborative recommender system~\cite{reco} to obtain ratings for all movies by every user. We cluster the movies into $5$ clusters using their vector of $18$ genres using spectral clustering so that each movie gets a unique cluster label.
  
% We solve the diverse matching problem using both negative cycle detection algorithm, and MIQP approaches for 1500 movies and match each user with three movies. The number of users is increased in steps of 50 to compare the timing performance of our approach to MIQP. For MIQP, we set a maximum run time of two hours (7200 seconds), at which we report the current best MIQP solution.

% Table~\ref{tab:res} shows that for all cases with the number of movies greater than 75, MIQP does not converge within two hours, while our method finds the optimum solution in lesser time. Interestingly, MIQP current solutions are found to be the same as the optimum solution found by our method. This shows that for this application, MIQP was able to search the solution but it was not able to prove that the solution is optimum. In contrast, our method finds the solution faster as well as guarantees that it is optimum.
  
%   %%Results
%   %% 1) 3883 MOVIES and 6040 users. We fix number of clusters to be 5. Each user wants 5 recommendations. We increase number of users from 50 to 500.
%   %% 2) Crowdwork: 
  
% %   \begin{equation*}
% %       \begin{aligned}
% % & \underset{S \in \mathcal{S}}{\text{minimize}}
% % & & \sum_{j \in Left}{f_j(S_j)} \\
% % \end{aligned}
% %   \end{equation*}
  
% %\subsection{Application to Crowdwork}

% \begin{table}[!htbp]
% \small
% \centering
% \begin{tabular}{ccc}
% \toprule
% %Number of movies & MIQP Time & Our Method Time & MIQP Objective & Our Method Objective & WBM Objective\\
% Number of movies & MIQP Time (s) & Our Method Time (s)\\
% \midrule
% 50 & 133 & 33\\
% 75 & 7200 & 98\\
% 100 & 7200 & 247\\
% 125 & 7200 & 663\\
% 150 & 7200 & 1069\\
% 175 & 7200 & 2581\\
% 200 & 7200 & 2316\\
% 250 & 7200 & 4609\\
% % 300 & 7200 & 9801\\
% \bottomrule\\
% \end{tabular}
% \caption{Comparison of MIQP and our method for MovieLens.}
% \label{tab:res}

% \end{table}



==> On Diverse Bipartite b-Matchings/general_weights.tex <==
\section{Diverse Weighted Bipartite $b$-Matching}\label{sec:general-weights}
In this section, we extend our algorithm to solve the case where the cost of assigning workers from the \emph{same} country to a team can be different. First, in each switch we put input and output ports for each worker. Inside each switch, there is a complete bipartite graph from input ports to the output ports. Consider an edge between an input port to an output port corresponding to workers $x_i$ and $x_j$. Per each feature $f_k$ where $x_i, x_j$ have the same values for $f_k$, $-2\lambda_k$ is added to the weight of the edge between $x_i, x_j$.
% This weight function ensures if $x_{j_1}$ is assigned to $T_i$ and $x_{j_2}$ is moved out of it, the diversity of $T_i$ does not change if $x_{j_1}$ and $x_{j_2}$ are from the same country, but it changes otherwise.

 Consider an edge from output port $x_{k}^{i_1}$ of switch $T_{i_1}$ to input port $x_{k}^{i_2}$ of switch $T_{i_2}$, where $x_{k}\in V_j$. The weight of this edge is equal to the change in the objective function by moving one worker from $V_j$ out of $T_{i_1}$, and adding that worker to $T_{i_2}$.
%If one of the switches is $T_0$, we don't add the changes made to the objective function by adding one person to $T_0$ or removing one person from $T_0$
The proof of the following theorem is similar to Thm.~\ref{thm:running-time}.
\begin{theorem}
The running time of the algorithm for general weights is $\mathcal{O}((\lambda_{max}\cdot |\mathcal{F}|\cdot n^2+\lambda_0U)\cdot n^2\cdot t^2(n+t))$, where $U$ is the maximum cost of any feasible $b$-matching.
\end{theorem}

==> On Diverse Bipartite b-Matchings/introduction.tex <==
\section{Introduction}
The bipartite matching problem occurs in many applications such as healthcare, advertising, and general resource allocation. Weighted bipartite $b$-matching is a generalization of this problem where each node on one side of the market can be matched to many items from the other side, and where edges may also have associated real-valued weights. Examples of weighted bipartite $b$-matching include assigning children to schools~\cite{drummond2015sat,kurata2017controlled}, reviewers to manuscripts~\cite{charlin2013toronto,Liu:2014:RMP:2645710.2645749}, and donor organs to patients~\cite{Dickerson:2015:FCH:2887007.2887094,Bertsimas19:Balancing}.

\citen{Ahmed:2017:DWB:3171642.3171649} introduced the notion of \textit{diverse} bipartite $b$-matching, where the goal was to simultaneously maximize the ``efficiency'' of an assignment along with its ``diversity.'' For example, a firm might want to hire several highly-skilled workers, but if that firm also cares about diversity it may want to ensure that some of those hires occur across marginalized categories of employees. They proposed an objective which combined economic efficiency and diversity demonstrating that, in practice, reducing the efficiency of a matching by small amounts can often lead to significant gains in diversity across a matching. However, their formulation was limited to diversity for a single feature. It also relied on solving a general Mixed-Integer Quadratic Program (MIQP), which is flexible but computationally intractable.

% \begin{figure}[ht!]
%     \centering
%     \includegraphics[width=0.23\textwidth]{figures/wbm.png}
%         \includegraphics[width=0.23\textwidth]{figures/dwbm.png}
%     \caption{An illustrative example of a non-diverse (left) versus diverse (right) matching; here, the diverse matching creates teams with workers from each country.}
%     \label{fig:matrix}
% \end{figure}

\begin{figure}[ht!]
    \centering
    \includegraphics[width=0.46\textwidth]{figures/gender_country.png}
    \caption{An illustrative example of single feature diverse matching (left) versus multi-feature diverse matching (right); here, the matching creates teams with workers from each country and gender.}
    \label{fig:matrix}
\end{figure}

In this work, we generalize the diverse matching problem and 
introduce matchings where each worker has \emph{multiple} features (e.g., country of origin, gender) and our goal is to form diverse teams with respect to all these features. We found that the problem with a single feature, studied by~\citen{Ahmed:2017:DWB:3171642.3171649}, can be reduced to a minimum quadratic cost maximum flow formulation and solved in polynomial time by an existing algorithm~\cite{Minoux1986}. In contrast, we provide NP-hardness results for the general case of multiple features.
%In this work, we study the diverse matching problem but develop an algorithm (and extensions) that is guaranteed to find the global optimum of the diverse, weighted, bipartite $b$-matching problem. Our method is also faster than the approach proposed by~\citen{Ahmed:2017:DWB:3171642.3171649} on the real-world benchmark test cases that they used. 
%We also propose two practical extensions of the problem. First, where each worker has multiple features (country of origin, gender) and our goal is to form diverse teams for all these features.  Second, where
%each task has a requirement of certain skills and workers are endowed with particular skills, which applies to the crowdsourcing setting. 


\noindent\textbf{Our contributions.}
The paper's main contributions follow:
\setlist{nolistsep}
\begin{itemize}[noitemsep,leftmargin=*]

    \item We provide the first pseudo-polynomial time algorithm for the diverse bipartite $b$-matching w.r.t.\ multiple features problem with class-specific weights.\footnote{That is, under conditions when the cost of assigning all items from one category to an item on the other side of the graph is the same. This holds when, e.g., one is matching academic papers to reviewers where each reviewer can specify exactly one field of expertise and the cost of assigning a paper to any of the reviewers \emph{within} the same field is the same but differs \textit{across} fields.} The key insight lies in detecting \emph{negative cycles} in an auxiliary graph representation, which we use to either provide incremental improvements to the incumbent diverse matching or prove that our negative-cycle-detection algorithms have found a globally-optimal matching. We also provide a general MIQP formulation for this problem.
        \item We then extend the algorithm to the diverse bipartite $b$-matching problems with \textit{general} edge weights, where edge weights of nodes within a category can be different.
        %\item  Next, we define a new variation of diverse $b$-matching problem where instead of considering only one feature for each worker, here country of citizenship, each worker has a set of features, and the diversity of a $b$-matching is calculated based on the set of all the features. We show how to extend our algorithm to capture this case as well.
        %\item In the next step, we extend our algorithm to a more general version of this problem, where each team has a vector of demands corresponding to a specific skill. Each worker has a specific skill. The goal is to find a diverse $b$-matching satisfying the vector of demands for each team.
    \item Lastly, we demonstrate our algorithm's applicability to paper-reviewer matching. Our algorithm takes less time to converge to an optimal solution than the proposed MIQP approach (using a state-of-the-art commercial solver). 
    
\end{itemize}

==> On Diverse Bipartite b-Matchings/multiple_attributes.tex <==
\section{Workers with Multiple Features}
\label{sec:multi-attributes}
In this section, we consider the diverse matching problem, however, instead of having only one feature for each worker (country of origin), there is a vector of features. An example of a feature set could be country of citizenship and gender. Let $F = \{f_1,\cdots, f_{|F|}\}$ denote the feature set for the workers.
In this case, the goal is to minimize $\lambda_{|F|+1}TU+\sum_{k=1}^{|F|}\lambda_k D_k$, where $D_k$ shows the diversity w.r.t the feature $f_k$. 

In the following, we show how to extend our framework to solve this problem. Assume the workers have two features $X,Y$, where $X$ could get any of the values $X_1, X_2$, and $Y$ could get any of the values $Y_1, Y_2$. In the graph representation, there is a switch per each team, and each switch has an input port and an output port per each possible combination of features (in this example the possible combinations of features are $\{(X_1,Y_1), (X_2, Y_1), (X_1, Y_2), (X_2, Y_2)\}$). Between two switches $T_{i_1}, T_{i_2}$, there is a directed edge from an output port of $T_{i_1}$, to an input port of $T_{i_2}$, if and only if the ports are corresponding to the same combination of features. The weight of this edge denotes the change in the objective function corresponding to one exchange. 

Inside a switch $T_i$, there is a directed edge from each input port to each output port. If the directed edge is connecting two ports such that their corresponding combinations of features have no value in common, the weight of this edge is equal to zero. Otherwise, per each feature $f_k$ that has the same value, $-2\lambda_k$ is added to this edge. For example, if there is an edge in $T_i$ from the input port corresponding to $(X_1,Y_1)$ to the output port $(X_1, Y_2)$, the weight of this edge is equal to $-2\lambda_1$.  
By applying a similar negative cycle detection algorithm, the optimum solution could be found. In the supplemental material, a sketch of the proof of optimality of the algorithm is given.
%The algorithm is similar to what we had before. First, we find an initial assignment. After that, in each iteration while there are negative cycles in the corresponding graph, a local exchange operation corresponding to the negative cycle is done. At the end, using a similar proof, it can be shown that the algorithm does not get stuck in a local optima and finds the global optimum. In the supplemental material, a sketch of the proof of optimality is given.





==> On Diverse Bipartite b-Matchings/prelims.tex <==
\section{Preliminaries}
\label{sec:prelim}
In this section, we first define the preliminaries for a diverse matching problem, where workers are to be matched to teams and each team wants workers belonging to a diverse set of features.
In our problem, we are given a set of features for the workers. Let $\mathcal{F} = \{f_1,\cdots, f_{|\mathcal{F}|}\}$ denote the feature set for the workers. An example of a feature set could be \{country of citizenship, gender\}. Each feature $f_k\in \mathcal{F}$ has one of the values $\mathcal{F}_k = \{f_{k,1},\cdots,f_{k, |\mathcal{F}_k|}\}$. Let $|\mathcal{F}_{k,k'}|$ denote the number of workers having value $f_{k,k'}$ for feature $f_k$.
%In this case, the goal is to minimize $\lambda_{|F|+1}TU+\sum_{k=1}^{|F|}\lambda_k D_k$, where $D_k$ shows the diversity w.r.t the feature $f_k$. 
%$\mathcal{C}=\{C_1,\ldots,C_m\}$ and each country $C_j$ has $|C_j|$ workers inside it. 
The set of workers is denoted by $X=\{x_1,\ldots,x_n\}$. We wish to form a set of teams $\{T_1,\ldots,T_t\}$ of the workers where each team $T_i$ has a demand of $d_i$, specifying the number of workers that need to be assigned to it. Each worker can be assigned to exactly one team. %The cost of assigning each worker from country $C_j \in \{C_1,\ldots,C_m\}$ to the team $T_i$ is denoted by $u_{i,j}$. We assume all costs are integers. 

The diversity of an assignment is denoted by $D$ and is equal to $\sum_{k=1}^{|\mathcal{F}|} \lambda_k D_k$, where $D_k$ shows the diversity w.r.t.\ feature $f_k$, and $\lambda_k\in \mathcal{Z}^+$ is a constant. Let $c_{i,k,k'}$ denote the number of workers in $T_i$ having value $f_{k,k'}\in \mathcal{F}_k$ for feature $f_k$. Then, $D_k = \sum_{i=1}^t\sum_{k'=1}^{|\mathcal{F}_k|}c_{i,k,k'}^2$.
To facilitate explanation, we assume throughout this paper that the country of origin is the $1$st feature, therefore, the number of workers assigned to team $T_i$ from $j$-th country is denoted by $c_{i,1,j}$. The cost of assigning each worker from $j$-th country to team $T_i$ is denoted by $u_{i,j}\in \mathcal{Z}^+$. We assume all costs are integers. The total cost of an assignment is $TU = \sum_{i=1}^t \sum_{j=1}^{|\mathcal{F}_1|} u_{i,j}\cdot c_{i,1,j}$.

% For example, diversity of an assignment w.r.t the countries is equal to $\sum_{i=1}^t \sum_{j=1}^m c_{i,j}^2$.
Our goal is to minimize the objective function which is equal to $\lambda \cdot D + \lambda_0 \cdot TU$, where $\lambda\in \mathcal{Z^+}^{|\mathcal{F}|}$, and $\lambda_0 \in \mathcal{Z^+}$ is a constant. Next, we provide Theorem \ref{thm:NP-completeness-multiple-features}, which shows that this problem is NP-hard.
%\saba{Where should we put the following theorem?}
\begin{theorem}
\label{thm:NP-completeness-multiple-features}
Minimizing the supermodular diversity function w.r.t multiple features is NP-hard.
\end{theorem}
\begin{proof}
We show a reduction from the \threecolor{} problem which is as follows: given a graph $G=(V,E)$ with $n$ vertices, does there exist a coloring with $n_1$ vertices of color $c_1$, $n_2$ vertices of color $c_2$, and $n_3$ vertices of color $c_3$, such that no two adjacent vertices receive the same color, and all the vertices are colored?

The reduction is as following: In \threecolor{}, assign a feature $f_k$ to each edge $e_k = (v_{k_1},v_{k_2})\in E$, and a worker to each vertex. Let $f_{k,i}$ denote the value of $f_k$ for the worker corresponding to $v_i\in V$. Let $f_{k,i} = i$ if $i\neq k_1, k_2$. Otherwise, let $f_{k,i}=0$.
%Each vertex $v_i\in V$ is mapped to a worker.
%and has a set of features $S_i$ that includes all the feature values corresponding to the edges that are incident on $v_i$. 
The goal is to form three teams $T_1, T_2, T_3$ with demands $d_1 = n_1, d_2 = n_2, d_3 = n_3$, respectively. We assume that all the costs of assigning workers to the teams are zero, therefore the objective function is to minimize the total diversity. Consider an arbitrary edge $e_k = (v_{k_1}, v_{k_2})$. If the endpoints of $e_k$ belong to different teams, $f_k$ contributes $n_1+n_2+n_3$ to the objective function since all the workers inside a team have different values for $f_k$. Otherwise, it contributes $n_1+n_2+n_3-2+2^2$ since workers corresponding to $v_{k_1}, v_{k_2}$ are the only workers having the same value for $f_k$ inside a team.
If the cost of the optimal solution for the diverse matching problem is $(n_1+n_2+n_3)\cdot|E|$, there does not exist a pair of workers in a team where the vertices corresponding to them are neighbouring in $G$. Otherwise if the cost of the optimal solution is more than $(n_1+n_2+n_3)\cdot|E|$, the \threecolor{} instance is infeasible.
\end{proof}

%We assume $\lambda$ is a rational number and $\lambda = \frac{\lambda_1}{\lambda_2}$ where $\lambda_1,\lambda_2\in \mathcal{Z^+}$. 
%We also assume $\lambda_1, \lambda_2$ are constants.
%Minimizing $\lambda \cdot D + TU$ is equivalent to minimizing $f~=~\lambda_1 \cdot D + \lambda_2\cdot TU$ and we use this new objective function when explaining the algorithm.

%In \S\ref{sec:general-weights}, we show how to generalize this algorithm to solve the problem for the case that the costs of assigning workers from the same country to a team could be different. We call that diverse bipartite $b$-matching with general weights.


%In \S\ref{sec:multi-attributes}, another generalization of this problem is introduced, where each worker has a vector of features, which is denoted with $F = \{f_1,\cdots, f_{|F|}\}$, for example $F = \{country, gender\}$. The goal is to minimize $\lambda_{|F|+1}TU+\sum_{k=1}^{|F|}\lambda_k D_k$, where $D_k$ shows the diversity w.r.t the feature $f_k$.

%In \S\ref{sec:skilled_workers}, there is a further assumption that each worker has a specific skill from the set  $S=\{s_1,\cdots,s_{|S|}\}$. Each team $T_i$ has a demand $d_{i,k}$ for each skill $s_k$. We show how to extend this framework to find a diverse bipartite $b$-matching which satisfies the skills demands for each team.


We are interested in solving this NP-hard problem. We begin by presenting two different representations of instances of the problem: one in matrix form (used for expositional ease), and the other in graph form (used to build our optimal diverse matching algorithm in Section~\ref{algorithm}). %we first represent it using an auxiliary graph representation. Next, 

\textbf{Matrix Representation:}

%In this representation, each column corresponds to a country, and each row corresponds to a team. Entry $c_{i,j}$ shows the number of workers from the country $C_j$ assigned to the team $T_i$.
%We introduce team $T_0$ as a dummy team, and $c_{0,i}$ shows the number of workers from country $C_i$ which are not assigned to any team. An example of matrix representation with three teams and two countries is shown in Fig.~\ref{fig:matrix-exchange}.

An example of matrix representation with three teams and two countries and two genders is shown in Fig.~\ref{fig:matrix-exchange}. In this representation, each column $V_j$ corresponds to a feature set $v_j = \{v_{j,1}, \cdots, v_{j,|\mathcal{F}|}\}$, where $\forall 1\leq k\leq|\mathcal{F}|, v_{j,k} \in \mathcal{F}_{k}$.
Each row corresponds to a team. Entry $w_{i,j}$ shows the number of workers with feature set $v_j$ assigned to $T_i$. We introduce a \emph{dummy team} $T_0$, and $w_{0,j}$ shows the number of workers with feature set $v_j$ who are not assigned to any team. 

\textbf{Matching Representation:}
In this representation, a bipartite graph $G=(\mathcal{X}\cup \mathcal{T}, E)$ is given. The nodes in $\mathcal{X}$ correspond to the workers, and are partitioned into $|\mathcal{V}|$ subsets $V_1,\cdots, V_{|\mathcal{V}|}$, where each subset corresponds to the feature set for a column in the matrix representation. Each vertex in $\mathcal{T}$ corresponds to one team. The assignment of workers to teams forms a $b$-matching, where the degree of node $T_i\in \mathcal{T}$ is $d_i$, and the degree of node $x\in \mathcal{X}$ is at most one.

\textbf{Local Exchange:} 
A local exchange happens when a group of teams decides to transfer one or more workers between each other while maintaining the total number of workers in each of them.
The exchange is done in a way that the initial demands of all the teams are fulfilled. 
Arrows in Fig.~\ref{fig:matrix-exchange} show a local exchange in a matrix representation. 

In this exchange, one worker from $V_2$ is moved from $T_3$ to $T_1$. Two workers from $V_1$ are moved. One is moved from $T_1$ to $T_2$, and the other one is moved from $T_2$ to $T_3$. The set of edges of local exchange in a matrix representation is called a cycle. The source-transitions of a cycle are the cells without any input edges, and the sink-transitions are the cells without any output edges. In Fig.~\ref{fig:matrix-exchange}, the nodes corresponding to $w_{3,2}$ and $w_{1,1}$ are source-transitions nodes, and the nodes corresponding to $w_{1,2}$ and $w_{3,1}$ are sink-transition nodes.

Figure~\ref{fig:matching-exchange} shows the same local exchange operation using a matching representation. In this figure, the black matching shows the initial assignment, and the dotted red matching shows the assignment after the exchange operation is done.

\begin{figure}
    \centering
    \includegraphics[width=0.30\textwidth]{figures/IJCAI-pic5v5.png}
    \caption{Matrix representation of three teams and workers from two countries and two genders. Dummy team $T_0$ accommodates unassigned workers. Arrows represent a local exchange.}
    \label{fig:matrix-exchange}
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{figures/IJCAI-pic9v1.png}
    \caption{Matrix representation embedding w.r.t country.}
    \label{fig:embedding-country}
\end{figure}

\begin{figure}
    \centering
        \includegraphics[width=0.3\textwidth]{figures/IJCAI-pic10v1.png}
    \caption{Matrix Representation Embedding w.r.t to gender.}
    \label{fig:embedding-gender}
\end{figure}


\begin{figure}
    \centering
        %\includegraphics[width=0.37\textwidth]{figures/IJCAI-pic4v3.png}
        \includegraphics[width=0.37\textwidth]{figures/figure5.pdf}
    \caption{Local exchange operation (in matching representation).}
    \label{fig:matching-exchange}
\end{figure}

\textbf{Gain of a local exchange: } 
Our goal is to minimize the objective function $f$, by doing some local exchanges. To find out, we first calculate the marginal gain from a given exchange operation which is the difference between the objective values before and after a local exchange. 
%For example, gain of the local exchange in Figure~\ref{fig:matrix-exchange} is $\Delta(\lambda_0\cdot TU + \lambda_1 D_1 + \lambda_2 D_2)$. 
In order to simplify this concept, we use the following definition:

\textbf{Embedding of Matrix Representation:}
Consider a given matrix representation $M$, it can be embedded into a matrix $M_{k}$ for a fixed feature $f_k$ in the following way: all the columns in $M$ corresponding to the same value $f_{k,k'}$ of $f_k$, are combined into a single column in $M_{k}$. For example, embedding of the matrix representation in Figure~\ref{fig:matrix-exchange} into $M_1, M_2$ w.r.t. the features country and gender are shown in Figures~\ref{fig:embedding-country} and \ref{fig:embedding-gender}.
Since in $M_1$, the number of people assigned from each country to each team is not changed, $\Delta(\lambda_0\cdot TU + \lambda_1 D_1) = 0$. Accoridng to $M_2$, $\Delta(\lambda_2 D_2) = \lambda_2\big((c_{3,2,2}-1)^2-(c_{3,2,2})^2+ (c_{1,2,2}+1)^2-(c_{1,2,2})^2+(c_{1,2,1}-1)^2-c_{1,2,1}^2+ (c_{3,2,1}+1)^2-c_{3,2,1}^2\big)$.
%, where $c_{i,k,k'}$ denotes the number of workers in $T_i$ having value $f_{k,k'}$ for feature $f_k$.

%$\lambda_1\big((c_{3,2}-1)^2-(c_{3,2})^2+ (c_{1,2}+1)^2-(c_{1,2})^2+(c_{1,1}-1)^2-c_{1,1}^2+ (c_{3,1}+1)^2-c_{3,1}^2\big)+\lambda_2\big(-u_{3,2} +u_{1,2}
%-u_{1,1}+u_{3,1}\big)$.
%(c_{3,1,1}-1)^2 - c_{3,1,1}^2 + (c_{1,1,1}+1)^2 - c_{1,1,1}^2
It can be seen that the contribution of the nodes which are not source-transition or sink-transition to the gain of a local exchange is zero (all the nodes in the local exchange in Figure~\ref{fig:embedding-country}, and the node corresponding to $c_{2,2,1}$ in $M_2$). If the net gain, i.e. $\Delta(\lambda_0\cdot TU + \lambda_1 D_1 + \lambda_2 D_2)$, is negative, then the local exchange can be considered beneficial and we can transfer the workers.

==> On Diverse Bipartite b-Matchings/related.tex <==
\section{Related Work}
%\saba{TODO: Minoux's result is not cited yet, but it is added to the bibfile (Minoux1986).}
%\saba{TODO: Graph alg is not motivated.}
Matching people to form diverse teams leverages the intersection of two past areas of research: the role of team diversity in collaborative work and how diversity among groups of resources is measured and used to form/match teams. Compared to related work, this paper provides a practical, high-performing method to perform diverse $b$-matching that can enable applications like diverse team formation or diverse resource allocation. Below we will use the example of diverse team formation (for example, in project teams within a company) to provide a concrete example to place prior work in context; however, our proposed approach is generally applicable to any diverse matching problem.

In the example of forming teams, the traditional approach is to use weighted bipartite $b$-matching (WBM) methods~\cite{basu2015task}. 
These methods maximize the total weight of the matching while satisfying some constraints. However, there are two major issues with these approaches. First, it assumes that the value provided by a person in a team is always fixed and independent of who else is in the team. This assumption may not hold in many cases. A new team member may provide more added value to the team if she is added to a smaller team compared to the case if she is added to a larger team. This property of diminishing marginal utility can be mathematically captured by a family of functions called submodular functions. Second, existing approaches do not account for diversity \textit{within} a team, where teams with workers from different backgrounds may be desirable. For example, different types of worker diversity have a direct impact on the success rate of tasks~\cite{ross2010crowdworkers}. Likewise, firms with a higher number of employees with higher education and diversity in the types of educations have a higher likelihood of innovating~\cite{ostergaard2011does} and increasing revenue for firms~\cite{hunt2015diversity}. In this paper, we address both these issues.

Past researchers have generally measured diversity by defining some notion of \textit{coverage}\textemdash that is, a diverse set is one that covers the space of available variation. Mathematically, researchers have done so via the use of \textit{submodular functions}, which encode the notion of diminishing returns~\cite{lin2012learning}; that is, as one adds items to a set that are similar to previous items, one gains less utility if the existing items in the set already ``cover'' the characteristics added by that new item. For example, many previous diversity metrics used in the information retrieval or search communities---including Maximum Marginal Relevance (MMR)~\cite{carbonell1998use} and Determinantal Point Processes~\cite{kulesza2012determinantal}---are instances of submodular functions. These functions can model notions of coverage, representation, and diversity~\cite{ahmed2018ranking} and they have been shown to achieve top results on common automatic document summarization benchmarks\textemdash \eg, at the Document Understanding Conference~\cite{lin2012learning}. %These functions are widely used in extractive document summarization~\cite{Lin11:Class} to get a diverse high-quality summary of documents.

Within matching, our work is closest to that of~\citen{Ahmed:2017:DWB:3171642.3171649}, which used a supermodular function to propose a diverse matching optimization method. Other researchers have also approached similar problems, with diversity either as an objective or as a constraint. For instance,~\citen{golz2018migration} match migrants to localities in a way that maximizes the expected number of migrants who find employment. \citen{benabbou2018diversity} study the trade-off between diversity and social welfare for the Singapore housing allocation. They model the problem as an extension of the classic assignment problem, with additional diversity constraints. \citen{lian2018conference} solve the assignment problem when preferences from one side over the other side are given and both sides have capacity constraints. They use order weighted averages to propose a polynomial-time algorithm which leads to high quality and more fair assignments. \citen{Agrawal18:Proportional} show that a simple iterative proportional allocation algorithm can be tuned to produce maximum matching with high entropy.  
%Finally,~\cite{Anapolska18:Minimum} address a complementary problem in minimum color-degree matching, and give motivational complexity results.
Finally,~\citen{Kobren:2019:PML:3292500.3330899} proposed two fairness-promoting algorithms for the paper-reviewer matching problem. They demonstrate that their algorithm achieves higher utility compared to state of the art matching algorithms that optimize for fairness only. 
In contrast, our goal is to develop an algorithm for finding the optimal assignment which maximizes utility as well as diversity along multiple features as an objective---along with having constraints on workload. 

We define a utility function that can be tuned to balance the diversity and total weight of matching. The diversity function is inspired by the Herfindahl index~\cite{hirschman1964paternity}, which is a statistical  measure of concentration and commonly used in economics. We provide a new algorithm that models the problem using an auxiliary graph and uses a heuristic improvement of the negative cycle detection of Bellman-Ford by~\citen{Goldberg93aheuristic}\footnote{We used the negative cycle detection algorithm by~\citen{Goldberg93aheuristic}. \citen{Cherkassky93shortestpaths} compared the performance of multiple negative cycle detection algorithms, and the algorithm by~\citen{Goldberg93aheuristic} was one of the fastest.} to find negative cycles and cancel them on a new graph to obtain an optimal solution for the original problem.

==> multiple_attributes.tex <==
\section{Workers with Multiple Features}
\label{sec:multi-attributes}
In this section, we consider the diverse matching problem, however, instead of having only one feature for each worker (country of origin), there is a vector of features. An example of a feature set could be country of citizenship and gender. Let $F = \{f_1,\cdots, f_{|F|}\}$ denote the feature set for the workers.
In this case, the goal is to minimize $\lambda_{|F|+1}TU+\sum_{k=1}^{|F|}\lambda_k D_k$, where $D_k$ shows the diversity w.r.t the feature $f_k$. 

In the following, we show how to extend our framework to solve this problem. Assume the workers have two features $X,Y$, where $X$ could get any of the values $X_1, X_2$, and $Y$ could get any of the values $Y_1, Y_2$. In the graph representation, there is a switch per each team, and each switch has an input port and an output port per each possible combination of features (in this example the possible combinations of features are $\{(X_1,Y_1), (X_2, Y_1), (X_1, Y_2), (X_2, Y_2)\}$). Between two switches $T_{i_1}, T_{i_2}$, there is a directed edge from an output port of $T_{i_1}$, to an input port of $T_{i_2}$, if and only if the ports are corresponding to the same combination of features. The weight of this edge denotes the change in the objective function corresponding to one exchange. 

Inside a switch $T_i$, there is a directed edge from each input port to each output port. If the directed edge is connecting two ports such that their corresponding combinations of features have no value in common, the weight of this edge is equal to zero. Otherwise, per each feature $f_k$ that has the same value, $-2\lambda_k$ is added to this edge. For example, if there is an edge in $T_i$ from the input port corresponding to $(X_1,Y_1)$ to the output port $(X_1, Y_2)$, the weight of this edge is equal to $-2\lambda_1$.  
By applying a similar negative cycle detection algorithm, the optimum solution could be found. In the supplemental material, a sketch of the proof of optimality of the algorithm is given.
%The algorithm is similar to what we had before. First, we find an initial assignment. After that, in each iteration while there are negative cycles in the corresponding graph, a local exchange operation corresponding to the negative cycle is done. At the end, using a similar proof, it can be shown that the algorithm does not get stuck in a local optima and finds the global optimum. In the supplemental material, a sketch of the proof of optimality is given.




